A generalisation of the honeycomb dimer model to higher dimensions

Linde, Moore, and Nordahl introduced a generalisation of the honeycomb dimer model to higher dimensions. The purpose of this article is to describe a number of structural properties of this generalised model. First, it is shown that the samples of the model are in one-to-one correspondence with the perfect matchings of a hypergraph. This leads to a generalised Kasteleyn theory: the partition function of the model equals the Cayley hyperdeterminant of the adjacency hypermatrix of the hypergraph. Second, we prove an identity which relates the covariance matrix of the random height function directly to the random geometrical structure of the model. This identity is known in the planar case but is new for higher dimensions. It relies on a more explicit formulation of Sheffield's cluster swap which is made possible by the structure of the honeycomb dimer model. Finally, we use the special properties of this explicit cluster swap to give a new and simplified proof of strict convexity of the surface tension in this case.

==> figures/2d_data_height.tex <==
% !TEX root =  ../main.tex
% \cipher{0}{2}{5}
% \cipher{0}{3}{4}
% \cipher{0}{4}{6}
% \cipher{0}{5}{5}
%
\cipher{-5}{12}{4}
\cipher{-5}{13}{6}
\cipher{-4}{10}{6}
\cipher{-4}{11}{5}
\cipher{-4}{12}{4}
\cipher{-4}{13}{3}
\cipher{-3}{8}{5}
\cipher{-3}{9}{7}
\cipher{-3}{10}{6}
\cipher{-3}{11}{5}
\cipher{-3}{12}{4}
\cipher{-3}{13}{6}
\cipher{-2}{6}{4}
\cipher{-2}{7}{6}
\cipher{-2}{8}{5}
\cipher{-2}{9}{4}
\cipher{-2}{10}{6}
\cipher{-2}{11}{5}
\cipher{-2}{12}{7}
\cipher{-2}{13}{6}
\cipher{-1}{4}{6}
\cipher{-1}{5}{5}
\cipher{-1}{6}{7}
\cipher{-1}{7}{6}
\cipher{-1}{8}{5}
\cipher{-1}{9}{4}
\cipher{-1}{10}{6}
\cipher{-1}{11}{5}
\cipher{-1}{12}{4}
\cipher{-1}{13}{3}
\cipher{0}{2}{5}
\cipher{0}{3}{4}
\cipher{0}{4}{6}
\cipher{0}{5}{5}
\cipher{0}{6}{7}
\cipher{0}{7}{6}
\cipher{0}{8}{5}
\cipher{0}{9}{7}
\cipher{0}{10}{6}
\cipher{0}{11}{5}
\cipher{0}{12}{4}
\cipher{0}{13}{3}
\cipher{1}{0}{4}
\cipher{1}{1}{6}
\cipher{1}{2}{5}
\cipher{1}{3}{4}
\cipher{1}{4}{6}
\cipher{1}{5}{5}
\cipher{1}{6}{7}
\cipher{1}{7}{6}
\cipher{1}{8}{5}
\cipher{1}{9}{4}
\cipher{1}{10}{6}
\cipher{1}{11}{5}
\cipher{1}{12}{4}
\cipher{1}{13}{3}
\cipher{2}{-1}{5}
\cipher{2}{0}{7}
\cipher{2}{1}{6}
\cipher{2}{2}{5}
\cipher{2}{3}{4}
\cipher{2}{4}{6}
\cipher{2}{5}{5}
\cipher{2}{6}{7}
\cipher{2}{7}{6}
\cipher{2}{8}{5}
\cipher{2}{9}{4}
\cipher{2}{10}{3}
\cipher{2}{11}{5}
\cipher{2}{12}{4}
\cipher{2}{13}{3}
\cipher{3}{-1}{5}
\cipher{3}{0}{4}
\cipher{3}{1}{3}
\cipher{3}{2}{5}
\cipher{3}{3}{4}
\cipher{3}{4}{6}
\cipher{3}{5}{5}
\cipher{3}{6}{4}
\cipher{3}{7}{3}
\cipher{3}{8}{2}
\cipher{3}{9}{4}
\cipher{3}{10}{6}
\cipher{3}{11}{5}
\cipher{3}{12}{4}
\cipher{3}{13}{3}
\cipher{4}{-1}{5}
\cipher{4}{0}{4}
\cipher{4}{1}{6}
\cipher{4}{2}{5}
\cipher{4}{3}{4}
\cipher{4}{4}{3}
\cipher{4}{5}{5}
\cipher{4}{6}{4}
\cipher{4}{7}{3}
\cipher{4}{8}{5}
\cipher{4}{9}{4}
\cipher{4}{10}{3}
\cipher{4}{11}{2}
\cipher{4}{12}{1}
\cipher{4}{13}{3}
\cipher{5}{-1}{5}
\cipher{5}{0}{7}
\cipher{5}{1}{6}
\cipher{5}{2}{5}
\cipher{5}{3}{4}
\cipher{5}{4}{6}
\cipher{5}{5}{5}
\cipher{5}{6}{4}
\cipher{5}{7}{3}
\cipher{5}{8}{2}
\cipher{5}{9}{1}
\cipher{5}{10}{0}
\cipher{5}{11}{2}
\cipher{6}{-1}{5}
\cipher{6}{0}{4}
\cipher{6}{1}{6}
\cipher{6}{2}{5}
\cipher{6}{3}{4}
\cipher{6}{4}{3}
\cipher{6}{5}{5}
\cipher{6}{6}{4}
\cipher{6}{7}{3}
\cipher{6}{8}{2}
\cipher{6}{9}{1}
\cipher{7}{-1}{5}
\cipher{7}{0}{7}
\cipher{7}{1}{6}
\cipher{7}{2}{5}
\cipher{7}{3}{4}
\cipher{7}{4}{3}
\cipher{7}{5}{5}
\cipher{7}{6}{4}
\cipher{7}{7}{3}
\cipher{8}{-1}{5}
\cipher{8}{0}{4}
\cipher{8}{1}{3}
\cipher{8}{2}{5}
\cipher{8}{3}{4}
\cipher{8}{4}{3}
\cipher{8}{5}{5}
\cipher{9}{-1}{5}
\cipher{9}{0}{4}
\cipher{9}{1}{3}
\cipher{9}{2}{5}
\cipher{9}{3}{4}
\cipher{10}{-1}{5}
\cipher{10}{0}{4}
\cipher{10}{1}{3}
\cipher{11}{-1}{2}


==> figures/2d_data_height0.tex <==
% !TEX root =  ../main.tex
% \cipher{0}{2}{5}
% \cipher{0}{3}{4}
% \cipher{0}{4}{6}
% \cipher{0}{5}{5}
%
\cipher{-5}{12}{4}
\cipher{-5}{13}{6}
\cipher{-4}{10}{6}
\cipher{-4}{11}{5}
\cipher{-4}{12}{4}
\cipher{-4}{13}{3}
\cipher{-3}{8}{5}
\cipher{-3}{9}{7}
\cipher{-3}{10}{6}
\cipher{-3}{11}{5}
\cipher{-3}{12}{4}
\cipher{-3}{13}{6}
\cipher{-2}{6}{4}
\cipher{-2}{7}{6}
\cipher{-2}{8}{5}
\cipher{-2}{9}{4}
\cipher{-2}{10}{6}
\cipher{-2}{11}{5}
\cipher{-2}{12}{7}
\cipher{-1}{4}{6}
\cipher{-1}{5}{5}
\cipher{-1}{6}{7}
\cipher{-1}{7}{6}
\cipher{-1}{8}{5}
\cipher{-1}{9}{4}
\cipher{-1}{10}{6}
\cipher{0}{2}{5}
\cipher{0}{3}{4}
\cipher{0}{4}{6}
\cipher{0}{5}{5}
\cipher{0}{6}{7}
\cipher{0}{7}{6}
\cipher{0}{8}{5}
\cipher{1}{0}{4}
\cipher{1}{1}{6}
\cipher{1}{2}{5}
\cipher{1}{3}{4}
\cipher{1}{4}{6}
\cipher{1}{5}{5}
\cipher{1}{6}{7}
\cipher{2}{-1}{5}
\cipher{2}{0}{7}
\cipher{2}{1}{6}
\cipher{2}{2}{5}
\cipher{2}{3}{4}
\cipher{2}{4}{6}
\cipher{3}{-1}{5}
\cipher{3}{0}{4}
\cipher{3}{1}{3}
\cipher{3}{2}{5}
\cipher{4}{-1}{5}
\cipher{4}{0}{4}


==> figures/2d_data_lozenge.tex <==
% !TEX root =  ../main.tex
% \loza{0}{0}
% \loza{0}{2}
% \loza{1}{1}
% \loza{1}{2}
% \loza{4}{3}
% \lozb{0}{0}
% \lozb{-1}{2}
% \lozb{0}{2}
% \lozc{1}{3}
% \lozc{0}{5}
% \lozc{-1}{5}
% \lozc{-2}{5}
%
\loza{0}{0}
\loza{0}{2}
\loza{1}{1}
\loza{1}{2}
\loza{3}{0}
\loza{4}{-1}
\loza{3}{2}
\loza{4}{1}
\loza{4}{2}
\loza{4}{3}
\lozb{0}{0}
\lozb{-1}{2}
\lozb{0}{2}
\lozb{-1}{4}
\lozb{1}{2}
\lozb{0}{4}
\lozb{2}{2}
\lozb{1}{4}
\lozb{3}{2}
\lozb{2}{4}
\lozb{1}{-1}
\lozb{2}{-2}
\lozb{3}{0}
\lozc{1}{1}
\lozc{1}{2}
\lozc{1}{3}
\lozc{0}{5}
\lozc{-1}{5}
\lozc{-2}{5}
\lozc{-1}{7}
\lozc{-2}{7}
\lozb{2}{-3}
\lozb{3}{-4}
\lozc{0}{0}
\lozc{2}{-1}
\lozc{2}{0}
\lozb{5}{-4}
\lozb{4}{-3}
\loza{5}{-2}
\lozb{5}{-2}
\lozb{4}{-1}
\loza{6}{-1}
\loza{6}{1}
\loza{5}{2}
\loza{6}{2}
\loza{6}{3}
\loza{7}{3}
\loza{8}{3}
\loza{9}{3}
\loza{8}{0}
\loza{9}{0}
\loza{5}{6}
\loza{5}{7}
\loza{5}{8}
\loza{5}{9}
\loza{6}{6}
\loza{6}{7}
\loza{6}{8}
\loza{7}{6}
\loza{7}{7}
\loza{11}{-2}
\lozb{8}{0}
\lozb{9}{0}
\lozb{10}{0}
\lozb{11}{-2}
\lozb{9}{-3}
\lozb{10}{-3}
\lozb{7}{-2}
\lozb{7}{-4}
\lozb{6}{-1}
\lozb{8}{-4}
\lozc{7}{3}
\lozc{8}{3}
\lozc{9}{1}
\lozc{9}{0}
\lozc{8}{0}
\lozc{7}{0}
\lozc{7}{-1}
\lozc{6}{1}
\lozc{6}{2}
\lozc{6}{3}
\lozc{4}{1}
\lozc{4}{2}
\lozc{5}{-1}
\lozc{6}{-1}
\lozc{7}{6}
\lozc{6}{6}
\lozc{5}{6}
\lozc{4}{6}
\lozc{4}{5}
\lozc{2}{6}
\lozc{1}{7}
\lozc{1}{8}
\lozc{1}{9}
\lozc{1}{10}
\lozc{0}{11}
\lozc{0}{12}
\lozc{2}{5}
\lozb{8}{3}
\lozb{7}{3}
\lozb{6}{3}
\lozb{4}{3}
\lozb{5}{2}
\lozb{4}{6}
\lozb{3}{8}
\lozb{3}{7}
\lozb{2}{9}
\lozb{1}{8}
\loza{-2}{5}
\loza{-2}{7}
\loza{-2}{8}
\loza{-1}{7}
\loza{0}{7}
\loza{-1}{8}
\loza{1}{7}
\loza{1}{8}
\loza{3}{7}
\loza{3}{6}
\loza{4}{6}
\loza{4}{5}
\lozc{1}{5}
\lozc{0}{7}
\loza{-3}{11}
\loza{-4}{11}
\loza{-5}{11}
\loza{-4}{10}
\loza{-5}{10}
\loza{-6}{12}
\loza{-4}{12}
\loza{-4}{14}
\loza{-3}{13}
\loza{-3}{14}
\loza{0}{12}
\loza{-1}{12}
\loza{-1}{11}
\loza{-1}{10}
\loza{0}{11}
\loza{2}{11}
\loza{2}{12}
\loza{1}{12}
\lozb{1}{12}
\lozb{2}{12}
\lozb{0}{12}
\lozb{-1}{12}
\lozb{-4}{12}
\lozb{-3}{11}
\lozb{-2}{10}
\lozb{-1}{8}
\lozb{0}{7}
\lozb{6}{8}
\lozb{5}{9}
\lozb{5}{10}
\lozb{4}{11}
\lozb{4}{12}
\lozb{3}{13}
\lozb{-6}{12}
\lozb{-5}{11}
\lozb{-6}{13}
\lozb{-3}{7}
\lozb{-2}{8}
\lozb{-2}{5}
\lozc{3}{9}
\lozc{3}{10}
\lozc{3}{11}
\lozc{3}{12}
\lozc{2}{11}
\lozc{2}{12}
\lozc{2}{13}
\lozc{2}{14}
\lozc{1}{15}
\lozc{1}{16}
\lozc{-1}{15}
\lozc{0}{15}
\lozc{-2}{15}
\lozc{-3}{15}
\lozc{-3}{14}
\lozc{-3}{13}
\lozc{-3}{11}
\lozc{-1}{11}
\lozc{-1}{10}
\lozc{-4}{11}
\lozc{-4}{10}
\lozc{-5}{10}
\lozc{-4}{8}
\lozc{-6}{14}
\lozc{-6}{15}
\lozc{-7}{16}


==> figures/2d_data_lozenge0.tex <==
% !TEX root =  ../main.tex
% \loza{0}{0}
% \loza{0}{2}
% \loza{1}{1}
% \loza{1}{2}
% \loza{4}{3}
% \lozb{0}{0}
% \lozb{-1}{2}
% \lozb{0}{2}
% \lozc{1}{3}
% \lozc{0}{5}
% \lozc{-1}{5}
% \lozc{-2}{5}
%
\loza{0}{0}
\loza{0}{2}
\loza{1}{1}
\loza{1}{2}
\loza{3}{0}
\loza{4}{-1}
\loza{3}{2}
\lozb{0}{0}
\lozb{-1}{2}
\lozb{0}{2}
\lozb{-1}{4}
\lozb{1}{2}
\lozb{0}{4}
\lozb{2}{2}
\lozb{1}{4}
\lozb{3}{2}
\lozb{2}{4}
\lozb{1}{-1}
\lozb{2}{-2}
\lozb{3}{0}
\lozc{1}{1}
\lozc{1}{2}
\lozc{1}{3}
\lozc{0}{5}
\lozc{-1}{5}
\lozc{-2}{5}
\lozc{-1}{7}
\lozc{-2}{7}
\lozb{2}{-3}
\lozb{3}{-4}
\lozc{0}{0}
\lozc{2}{-1}
\lozc{2}{0}
\lozb{5}{-4}
\lozb{4}{-3}
\loza{5}{-2}
\lozb{5}{-2}
\lozb{4}{-1}
\lozc{2}{6}
\lozc{1}{7}
\lozc{1}{8}
\lozc{1}{9}
\lozc{2}{5}
\lozb{3}{8}
\lozb{3}{7}
\lozb{2}{9}
\lozb{1}{8}
\loza{-2}{5}
\loza{-2}{7}
\loza{-2}{8}
\loza{-1}{7}
\loza{0}{7}
\loza{-1}{8}
\lozc{1}{5}
\lozc{0}{7}
\loza{-3}{11}
\loza{-4}{11}
\loza{-5}{11}
\loza{-4}{10}
\loza{-5}{10}
\loza{-6}{12}
\loza{-4}{12}
\loza{-4}{14}
\loza{-3}{13}
\loza{-3}{14}
\loza{0}{12}
\loza{-1}{12}
\loza{-1}{11}
\loza{-1}{10}
\loza{0}{11}
\lozb{2}{12}
\lozb{0}{12}
\lozb{-1}{12}
\lozb{-4}{12}
\lozb{-3}{11}
\lozb{-2}{10}
\lozb{-1}{8}
\lozb{0}{7}
\lozb{6}{8}
\lozb{5}{9}
\lozb{5}{10}
\lozb{4}{11}
\lozb{4}{12}
\lozb{3}{13}
\lozb{-6}{12}
\lozb{-5}{11}
\lozb{-6}{13}
\lozb{-3}{7}
\lozb{-2}{8}
\lozb{-2}{5}
\lozc{-2}{15}
\lozc{-3}{15}
\lozc{-3}{14}
\lozc{-3}{13}
\lozc{-3}{11}
\lozc{-1}{11}
\lozc{-1}{10}
\lozc{-4}{11}
\lozc{-4}{10}
\lozc{-5}{10}
\lozc{-4}{8}
\lozc{-6}{14}
\lozc{-6}{15}
\lozc{-7}{16}


==> sections/120_surface_tension.tex <==
%!TEX root= ../main.tex

\section{The surface tension}
\label{sec:st}

\subsection{Definition and well-definedness}
If $f:H\to\mathbb R$ is Lipschitz then $\nabla f$ exists almost everywhere and takes values in $\mathcal S$.
The surface tension $\sigma(s)$ describes,
for each $s\in\mathcal S$, the asymptotics of the number of height functions
that approximate the slope $s$.
For $n\in\mathbb N$, let $B_n$ and $\bar B_n$ denote the subsets of $X^d$
defined by
\begin{equation}
  \label{eq:boxdef}
    B_n:=\{a_1\mathbf g_1+\dots+a_d\mathbf g_d:0<a_1,\dots,a_d<n\},\quad
    \bar B_n:=\{a_1\mathbf g_1+\dots+a_d\mathbf g_d:0\leq a_1,\dots,a_d\leq n\}.
\end{equation}
Note that $\bar B_n=B_{n+2}+\mathbf g_{d+1}$,
and that $|B_n|=(n-1)^d$ and $|\bar B_n|=(n+1)^d$.
The set $B_n$ is called the \emph{box of size $n$},
and $\bar B_n$ is called the \emph{closed box of size $n$},
as it contains both $B_n$ and all neighbours of vertices in $B_n$.

\begin{definition}
  \label{def:sigma_n}
  For each $s\in\mathcal S$ and $n\in\mathbb N$, write
  \[\sigma_n(s):=-n^{-d}\log \inf\nolimits_{a\in\mathbb R}|\Omega(B_n,\lfloor s+a \rfloor)|=-n^{-d}\log \inf\nolimits_{a\in[0,d+1)}|\Omega(B_n,\lfloor s+a \rfloor)|.\]
\end{definition}

Note that the two numbers in the definition are the same because
$|\Omega(R,f)|=|\Omega(R,f+d+1)|$ for any $R\subset X^d$
and $f\in\Omega$.
A bijection from the first set to the second is given by the map
 $g\mapsto g+d+1$.

\begin{lemma}
  \label{lemma:SurfaceTensionFirstExistence}
  For each $s\in\mathcal S$, the limit
$  \sigma(s):=\lim_{n\to\infty}\sigma_n(s)
$  exists and takes values in $[-\log 2,0]$.
\end{lemma}

\begin{definition}
  The function $\sigma:\mathcal S\to [-\log 2,0]$
   is called the \emph{surface tension}.
\end{definition}

The appearance of the number $a$ in Definition~\ref{def:sigma_n} makes
it easier to prove that the sequence $(\sigma_n(s))_{n\in\mathbb N}$
converges as $n\to\infty$.
We shall see later---in
Corollary~\ref{corollary:set_a_zero}---that we may equally well take $a=0$.
% Theorem~\ref{thm:seq_c_n} also shows that the definition of the surface tension is
% invariant under perturbing $\lfloor s\rfloor$.

For $R\subset X^d$, write $\partial R$ for the vertices of $X^d$
that are adjacent to---but not contained in---$R$.
If $f$ and $g$ are real-valued functions
defined on disjoint sets $R\subset X^d$
and $R'\subset X^d$ respectively,
then write $fg$ for the function
\[fg:R\cup R'\to\mathbb R,\,\mathbf x\mapsto \begin{cases}
f(\mathbf x)&\text{if $\mathbf x\in R$,}\\
g(\mathbf x)&\text{if $\mathbf x\in R'$.}
\end{cases}\]

\begin{remark}
  \label{rem:trivialIntermediate}
  We make some important observations before providing a proof to Lemma~\ref{lemma:SurfaceTensionFirstExistence}.
  \begin{enumerate}
    \item For any height function $f\in\Omega$, the set $\Omega(R,f)$
    is increasing in the choice of $R\subset X^d$.
    In particular, the cardinality $|\Omega(R,f)|$ is increasing in $R$.

    \item\label{secondpoint}
     Let $R\subset X^d$ be finite
    and $f$ a height function.
    The nontrivial behaviour of the set
    $\Omega(R,f)$ depends only on the choice of the set $R$ and on the values of
    $f$ on $\partial R$.
    To see why, note first that each function $g\in \Omega(R,f)$
    is characterised by its restriction $g|_R$;
     the values of $g$ on $R^\complement$
    are given by $f$.
    To determine if a real-valued extension $g$ of
     $f|_{R^\complement}$ to $X^d$ is a height function, we need to verify that the values
    of $\nabla g$ are correct on $E^d(R)$. This condition depends on $f|_{\partial R}$
    and $g|_{R}$ only
    because every edge in $E^d(R)$ is contained in $R\cup\partial R$.

    The following corollary is useful in practice.
    Suppose that $f$ and $g$ are height functions that differ by a constant
    on $\partial R$, say $(f-g)|_R=a\in (d+1)\mathbb Z$.
    Then the map
    \[
    \Omega(R,f)\to\Omega(R,g)
    ,\,
    h\mapsto g|_{R^\complement} (h-a)|_R
    \]
    is a bijection.
    In particular, $|\Omega(R,f)|=|\Omega(R,g)|$.


    \item
    Let $f$ denote a height function.
    Suppose that some finite set $R\subset X^d$ is not connected as a subset of $(X^d,E^d)$, say it is the disjoint union of $R_1$ and $R_2$,
    with no vertex of $R_1$ adjacent to a vertex of $R_2$.
    To check that some real-valued extension $g$ of $f|_{R\complement}$
    to $X^d$ is a height function,
    we must verify that $\nabla g$ takes the correct values on $E^d(R)$.
    But $E^d(R)$ is the disjoint union of $E^d(R_1)$ and $E^d(R_2)$,
    and therefore we may---for the sake of checking this condition---consider the values of $g$ on $R_1$ separately
    from the values of $g$ on $R_2$.
    In other words, the set of extensions of $f|_{R^\complement}$
    to $X^d$ decomposes as the product of the set of extensions to $R_1^\complement$
    and the set of extensions to $R_2^\complement$.

    Formally, we establish the following result.
    Let $f$ be a height function.
    Suppose that $R_1,R_2\subset X^d$ are finite, disjoint, and with no vertex of $R_1$
    adjacent to a vertex of $R_2$.
    Then the map
    \[\Omega(R_1,f)\times \Omega(R_2,f)\to \Omega(R_1\cup R_2,f),\, (g_1,g_2)\mapsto f|_{(R_1\cup R_2)^\complement} g_1|_{R_1} g_2|_{R_2}\]
    is a bijection.
    In particular, $|\Omega(R_1\cup R_2,f)|=|\Omega(R_1,f)|\cdot|\Omega(R_2,f)|$.
  \end{enumerate}
\end{remark}

\begin{proof}[Proof of Lemma~\ref{lemma:SurfaceTensionFirstExistence}]
  If $s\in \mathcal S$, $a\in\mathbb R$, and $\theta\in\Theta$,
  then it is straightforward to prove that
  $\tilde\theta \lfloor s+a\rfloor = \lfloor s + b\rfloor $
  for some $b\in \mathbb R$.
  This implies that
  $
    \tilde\theta\Omega(\theta B_n,\lfloor s+a\rfloor)
    =   \Omega( B_n,\tilde\theta\lfloor  s+a\rfloor)
    = \Omega( B_n,\lfloor s+b\rfloor)$.
The three sets have the same cardinality,
  and therefore
    \begin{equation}
      \label{eq:usefultranslationinvariance}
      \inf\nolimits_{a\in\mathbb R}|\Omega(\theta B_n,\lfloor s+a \rfloor)|=\inf\nolimits_{a\in\mathbb R} |\Omega(B_n,\lfloor s+a \rfloor)|:
    \end{equation}
  taking the infimum of the cardinalities over all $a\in\mathbb R$ resolves the absence of shift-invariance of $\nabla \lfloor s\rfloor$ that is a consequence
  of passing from $s$ to $\lfloor s\rfloor$.

  For any $n\in\mathbb N$ and any $a\in\mathbb R$ we have
  $1\leq |\Omega(B_n,\lfloor s+a \rfloor)|\leq 2^{|B_n|}\leq 2^{n^d}$,
  and consequently $-\log 2\leq \sigma_n(s)\leq 0$.
  Now
  $\inf_{a\in\mathbb R}|\Omega(B_n,\lfloor s+a \rfloor)|$
  is increasing in $n$, and therefore $\sigma_{n+1}(s)\leq (n/(n+1))^d \sigma_n(s)$ for every $n\in\mathbb N$.
  To prove that the sequence converges,
  it suffices to prove that $\sigma_{kn}(s)\leq \sigma_n(s)$ for any $n,k\in\mathbb N$.
  Remark~\ref{rem:trivialIntermediate} implies that
  \begin{align*}
    |\Omega(B_{kn},\lfloor s+a \rfloor)|
    &\geq
    |\Omega(\cup_{x\in \{0,\dots,k-1\}^d}(B_n+nx_1\mathbf g_1+\dots+nx_d\mathbf g_d),\lfloor s+a \rfloor)|\\
    &=\textstyle\prod_{x\in \{0,\dots,k-1\}^d}
    |\Omega(B_n+nx_1\mathbf g_1+\dots+nx_d\mathbf g_d,\lfloor s+a \rfloor)|
  \end{align*}
  and taking infima gives
  \begin{align*}
    \textstyle\inf_{a\in\mathbb R}|\Omega(B_{kn},\lfloor s+a \rfloor)|
    &\textstyle\geq \prod_{x\in \{0,\dots,k-1\}^d}
    \inf_{a\in\mathbb R}
    |\Omega(B_n+nx_1\mathbf g_1+\dots+nx_d\mathbf g_d,\lfloor s+a \rfloor)|\\
    &=\textstyle\inf_{a\in\mathbb R}
    |\Omega(B_n,\lfloor s+a \rfloor)|^{k^d}.
  \end{align*}
  This proves that $\sigma_{kn}(s)\leq\sigma_n(s)$ and therefore the lemma.
\end{proof}

% Suppose that
% $s\in\mathcal S$ is in the topological boundary
% of the set of Lipschitz slopes $\mathcal S$.
% This means that $s(\mathbf g_i)=1$ for some $i$,
% and therefore
%  $\nabla \lfloor s+a\rfloor (\mathbf x,\mathbf x+\mathbf g_i)=1$ for all $\mathbf x\in X^d$.
% There is no flexibility;
% it is not possible to find height functions
% that agree to $\lfloor s+a\rfloor$
% on all but a finite number of vertices of $X^d$.
% The set
% $\Omega(B_n,\lfloor s+a \rfloor)$ contains precisely one element:
% the original height function $\lfloor s+a \rfloor$ itself.
% The surface tension $\sigma(s)$ therefore equals zero for all $s\in\partial\mathcal S$.
% The function $\sigma$ is thus not strictly convex on the boundary of $\mathcal S$.
% The goal is to show that $\sigma$ is strictly convex on the interior of $\mathcal S$.

\subsection{Stability of the definition}
The crucial step in the previous lemma was the supermultiplicativity, which relies on Equation~\ref{eq:usefultranslationinvariance}.
The following theorem may be considered an alternative definition
of the surface tension, and it effectively dispenses
with the $a$ in Definition~\ref{def:sigma_n}.
(See Corollary~\ref{corollary:set_a_zero}.)

\begin{theorem}
  \label{thm:seq_c_n}
  Suppose that $n^{-1}\|f_n|_{\partial B_n}-s|_{\partial B_n}\|_\infty\to 0$ as $n\to\infty$ for some
  slope $s\in\mathcal S$ and some sequence of height functions $(f_n)_{n\in\mathbb N}\subset \Omega$.
  Then $\sigma(s)=\lim_{n\to\infty} -n^{-d}\log |\Omega(B_n,f_n)|$.
\end{theorem}

\begin{proof}
  We distinguish two cases,
  depending on wether or not $s\in\partial\mathcal S$.

  First consider the case that $s\in\partial\mathcal S$.
  We are going to show that
  $\lim_{n\to\infty} -n^{-d}\log |\Omega(B_n,f_n)|=0$.
  Therefore we only require an asymptotic upper bound
  on $|\Omega(B_n,f_n)|$.
  We obtain a sufficient combinatorial bound on $|\Omega(B_n,f_n)| $
  through a series of small intermediate results.
  There exists an $i$ such that $s(\mathbf g_i)=1$
  because $s\in\partial\mathcal S$.
  Fix a finite set $R\subset X^d$ and a height function $f$
  for now.
  Write $E^d(R)_i$ for the edges in $E^d(R)$
  of the form $\{\mathbf x,\mathbf x+\mathbf g_i\}$,
  and observe that $|R|\leq |E^d(R)_i|\leq |R|+|\partial R|$.
  \begin{enumerate}
    \item
    \emph{Each function $g\in\Omega(R,f)$ is characterised
    by the set $T(g)\cap E^d(R)_i$.}
    Fix $\mathbf x\in R$;
    we aim to recover
    $g(\mathbf x)$
    from $T(g)\cap E^d(R)_i$.
    Write $\mathbf p=(\mathbf p_k)_{0\leq k\leq n}$ for the shortest path
    that starts at $\mathbf x$,
    ends in $\partial R$,
    and with every increment of the form $\mathbf g_i$.
    Then the edges of $\mathbf p$ are in $E^d(R)_i$, and
    \[g(\mathbf x)=g(\mathbf p_n)-\int_\mathbf p\alpha_{T(g)}=f(\mathbf p_n)-\int_\mathbf p\alpha_{T(g)\cap E^d(R)_i}.\]
    This proves the claim.
    \item \emph{The number $|T(g)\cap E^d(R)_i|$
    is constant over all height functions $g\in\Omega(R,f)$.}
    To see that this is the case, observe simply that
    the number $|T(g)\cap E^d(R)_i|$ is stable under the local moves that were defined in Subsection~\ref{subsec:localmove}.
  \end{enumerate}
  The first two intermediate results imply jointly that
  \[|\Omega(B_n,f_n)|\leq {|B_n|+|\partial B_n| \choose |T(f_n)\cap E^d(B_n)_i|}.\]
  In order to bound $|\Omega(B_n,f_n)|$,
  we need to bound the two numbers in the binomial term on the right.
  For the number on top we observe simply that
  $|B_n|+|\partial B_n|\leq (n+1)^d$.
  \begin{enumerate}[resume]
    \item\emph{We have $\sum_{\mathbf x\in \partial B_n}|f_n(\mathbf x)-s(\mathbf x)|\geq (d+1)|T(f_n)\cap E^d(B_n)_i|$.}
    Associate to each $\mathbf x\in B_n$ the unique path $\mathbf p^\mathbf x$
    that starts and ends in $\partial B_n$, has all other
    vertices in $B_n$, travels through $\mathbf x$,
    and with all increments of the form $\mathbf g_i$.
    Write $\mathbf p_\pm^\mathbf x$ for the start- and endpoint of $\mathbf p^\mathbf x$.
    Write $P:=\{\mathbf p^\mathbf x:\mathbf x\in B_n\}$
    for the collection of all such paths.
    If we identify each path in $P$ with its set of traversed edges,
    then $P$ partitions $E^d(B_n)_i$.
    Each vertex in $\partial B_n$ is the start- or endpoint of at most one
    path in $P$.
    For each path $\mathbf p\in P$, we have---writing $|\mathbf p|$ for the
    length of $\mathbf p$---
    \[(f_n(\mathbf p_+)-f_n(\mathbf p_-))-(s(\mathbf p_+)-s(\mathbf p_-))=\int_\mathbf p\alpha_{T(f_n)}-|\mathbf p|=-(d+1)|T(f_n)\cap\mathbf p|.\]
    This implies that $|f_n(\mathbf p_-)-s(\mathbf p_-)|+|f_n(\mathbf p_+)-s(\mathbf p_+)|\geq (d+1)|T(f_n)\cap\mathbf p|$.
    Sum over all $\mathbf p\in P$ for
    \begin{align*}
      \sum_{\mathbf x\in \partial B_n}|f_n(\mathbf x)-s(\mathbf x)|
      &\geq \sum_{\mathbf p\in P}|f_n(\mathbf p_-)-s(\mathbf p_-)|+|f_n(\mathbf p_+)-s(\mathbf p_+)|
      \\&\geq \sum_{\mathbf p\in P} (d+1)|T(f_n)\cap\mathbf p|
      = (d+1)|T(f_n)\cap E^d(B_n)_i|.
    \end{align*}
    This is the claim.
    \item \emph{We have $(n+1)^{-d}|T(f_n)\cap E^d(B_n)_i|\to 0$ as $n\to\infty$.}
    To see that this limit is correct, observe that
    \begin{align*}
      (n+1)^{-d}(d+1)|T(f_n)\cap E^d(B_n)_i|&\leq (n+1)^{-d}
      \sum_{\mathbf x\in \partial B_n}|f_n(\mathbf x)-s(\mathbf x)|
      \\&\leq \frac{|\partial B_n|}{(n+1)^{d-1}}
      \frac{\|f_n|_{\partial B_n}-s|_{\partial B_n}\|_\infty}{n+1}\to 0
    \end{align*}
    as $n\to\infty$. In particular, the first fraction remains bounded as $n\to\infty$,
    and the second fraction tends to zero by assumption.
    This proves the claim.
  \end{enumerate}
  Conclude now that
  \[|\Omega(B_n,f_n)|\leq {\phantom {a_n}(n+1)^d \choose a_n (n+1)^d}\]
  for some sequence $(a_n)_{n\in\mathbb N}\subset (0,1)$ tending
  to $0$ as $n\to\infty$.
  It is straightforward to demonstrate that
  \[-\log |\Omega(B_n,f_n)|\geq -\log {\phantom {a_n}(n+1)^d \choose a_n (n+1)^d}\geq (n+1)^d (a_n\log a_n + (1-a_n)\log (1-a_n)).\]
  In particular,
  multiplying by $n^{-d}$ and taking $n\to\infty$ gives
  $\lim_{n\to\infty} -n^{-d}\log |\Omega(B_n,f_n)|=0$,
  as desired.

  The proof for $s$ in the interior of $\mathcal S$
  is different.
  It relies on Remark~\ref{rem:trivialIntermediate},
   the Kirszbraun theorem,
  and the fact that all slopes in a neighbourhood of $s$ are also Lipschitz.
  For the lemma it is sufficient to show that
  for any $0<\varepsilon<1/2$ there exists an $N\in\mathbb N$ such that
  for all $n\geq N$,
  \begin{equation}
    \label{eq:inequalitiestoprove}
\inf_{a\in\mathbb R}|\Omega(B_{n-2\lceil n\varepsilon\rceil},\lfloor s+a\rfloor)|\leq |\Omega(B_n,f_n)|\leq \inf_{a\in\mathbb R}|\Omega(B_{n+2\lceil n\varepsilon\rceil},\lfloor s+a\rfloor)|.
  \end{equation}
  Indeed, the inequalities imply that
  \[
  {\textstyle\left(\frac{n-2\lceil n\varepsilon\rceil}{n}\right)^d}
  \sigma_{n-2\lceil n\varepsilon\rceil}(s)
    \geq -n^{-d}\log |\Omega(B_n,f_n)|\geq {\textstyle\left(\frac{n+2\lceil n\varepsilon\rceil}{n}\right)^d} \sigma_{n+2\lceil n\varepsilon\rceil}(s)
  \]
  and taking limits gives
  \[
  (1-2\varepsilon)^d\sigma(s)\geq \limsup_{n\to\infty}-n^{-d}\log |\Omega(B_n,f_n)|
  \geq \liminf_{n\to\infty}-n^{-d}\log |\Omega(B_n,f_n)|
  \geq (1+2\varepsilon)^d\sigma(s),
  \]
  which implies the desired convergence because $\varepsilon$ may be taken arbitrarily small.
  It suffices to prove (\ref{eq:inequalitiestoprove})
  for fixed $0<\varepsilon<1/2$
  and $n\in\mathbb N$ sufficiently large.

  Fix $0<\varepsilon<1/2$ and $n\in\mathbb N$ large. We focus on the inequality on the right in (\ref{eq:inequalitiestoprove}), the other inequality is similar.
  Define $B_n^\varepsilon:=B_{n+2\lceil n\varepsilon\rceil}+\lceil n\varepsilon\rceil \mathbf g_{d+1}$,
  and recall from the proof of
   Lemma~\ref{lemma:SurfaceTensionFirstExistence}
  that
  \[
  \inf_{a\in\mathbb R}|\Omega(B_{n+2\lceil n\varepsilon\rceil},\lfloor s+a\rfloor)|
  =
  \inf_{a\in\mathbb [0,d+1)}|\Omega(B_n^\varepsilon,\lfloor s+a\rfloor)|.
  \]
  Recall that $\mathbf g_{d+1}=-(\mathbf g_1+\dots+\mathbf g_d)$
  and therefore
  \[
  B_n^\varepsilon =B_{n+2\lceil n\varepsilon\rceil}+\lceil n\varepsilon\rceil \mathbf g_{d+1}
  =
  \{a_1\mathbf g_1+\dots+a_d\mathbf g_d:-\lceil n\varepsilon\rceil<a_1,\dots,a_d<n+\lceil n\varepsilon\rceil\}.
  \]
  Conclude that $B_n\subset B_n^\varepsilon$
  and
  $d_{(X^d,E^d)}(\partial B_n,\partial B_n^\varepsilon)\geq  n\varepsilon$.

  Suppose now that there exists a height function $g$
  that equals $f_n$ on the boundary of $B_n$
  and that equals $\lfloor s+a\rfloor$ on the boundary of $B_n^\varepsilon$---for some fixed $a\in [0,d+1)$.
  Then Remark~\ref{rem:trivialIntermediate} says that
  \[|\Omega(B_n,f_n)|=|\Omega(B_n,g)|\leq |\Omega(B_n^\varepsilon,g)|
  =|\Omega(B_n^\varepsilon,\lfloor s+a\rfloor)|.\]
  To finish the proof of the lemma it suffices
  to show that, for $n$ sufficiently large, the function
  \[f_n|_{\partial B_n}  \lfloor s+a\rfloor |_{\partial B_n^\varepsilon}\] is
  Lipschitz for any $a\in [0,d+1)$; the Kirszbraun theorem then tells us that the desired extension $g$ exists.
  We already know that $f_n$ and $\lfloor s+a\rfloor$ are Lipschitz;
  it suffices to check that
  for $n\in\mathbb N$ sufficiently large the function
  $f_n|_{\{\mathbf x\}} \lfloor s+a\rfloor|_{\{\mathbf y\}}$
  is Lipschitz, for any $\mathbf x\in\partial B_n$, $\mathbf y\in\partial B_n^\varepsilon$, $a\in [0,d+1)$.
  This is straightforward to check because
  \begin{enumerate}
    \item $n^{-1}\|f_n|_{\partial B_n}-s|_{\partial B_n}\|_\infty\to 0$ as $n\to\infty$,
    \item $n^{-1}\|\lfloor s+a \rfloor|_{\partial B_n^\varepsilon} - s |_{\partial B_n^\varepsilon}\|_\infty\to 0$ as $n\to\infty$,
    \item $d_{(X^d,E^d)}(\partial B_n,\partial B_n^\varepsilon)\geq n\varepsilon$,
    \item $s$ is in the interior of $\mathcal S$: the set of Lipschitz slopes.
  \end{enumerate}
  In particular, (1) holds by hypothesis,
  and (2) is evident as $\|\lfloor s+a \rfloor - s|_{X^d}\|_\infty\leq d+1$ for $a\in [0,d+1)$.
\end{proof}

We state three immediate corollaries of (the proof of) the previous lemma.

\begin{corollary}
  \label{corollary:set_a_zero}
  For every $s\in\mathcal S$, we have $\sigma(s)=\lim_{n\to\infty}
  -n^{-d}\log |\Omega(B_n,\lfloor s \rfloor)|$.
\end{corollary}

 \begin{corollary}
   For every $s\in\partial\mathcal S$, we have $\sigma(s)=0$.
 \end{corollary}

\begin{corollary}
  The surface tension $\sigma:\mathcal S\to [-\log 2,0]$ is continuous.
\end{corollary}


==> sections/160_open_problems.tex <==
%!TEX root= ../main.tex
\section{Final remarks and open problems}
\label{sec:final}

\subsubsection*{Do other models allow for a similar analysis?}
The cluster boundary swap roots in
Lemma~\ref{twocomponents},
which in turn refers back to Lemmas~\ref{lem:cons}~and~\ref{important}.
Two ingredients are required to make the cluster boundary swap work.
First, one needs a graph, together with a set of base loops.
By a \emph{set of base loops}
we simply mean a collection of
 closed walks through the graph, such that a flow on the graph is conservative if and only if
the flow integrates to zero along each closed walk in that designated collection.
For example, if the graph is planar,
then the set of closed walks along faces
forms a set of base loops.
This replaces Lemma~\ref{lem:cons}.
Second, one needs to define the set of height functions $f$ by allowing
two options for the discrete derivative of $f$ on each edge---as in the defining Equation~\ref{hfdef}---such that each base loop has exactly one ``special''
edge
 in the sense of the uniqueness of the
 edge of Lemma~\ref{important},~\ref{important_two}.
An equivalent of Lemma~\ref{important},~\ref{important_three} and~\ref{important_four} then follows,
and one is ready to employ the cluster boundary swap.
In fact, the Kasteleyn theory and its generalisation depend on exactly the same uniqueness statement, as the special edge then
matches all the base loops that pass through it.
It seems that a clean level set decomposition
with cluster boundary swap is possible for exactly those models
that allow for a generalised Kasteleyn theory.
The author is not aware of any models satisfying the two conditions, other than planar dimer models and the model of the current paper. In particular, it is not known if such
 a random height functions model exists on the square lattice $\mathbb Z^d$ with $d\geq 3$.
For $d=2$ this is precisely the model of domino tilings.

\subsubsection*{Does the model exhibit a frozen region in any dimension?}
Of much interest in the original dimer model is the
frozen region \cite{jockusch1998random}.
It was conjectured in \cite{Linde} that the model of the current paper exhibits
a similar phenomenon.

\subsubsection*{The nature of the shift-invariant gradient Gibbs measures.}
If $d=2$,
then
 each slope $s\in\operatorname{Int}\mathcal S$ corresponds
to a unique ergodic gradient Gibbs measure $\mu$ of that slope \cite{kenyon2001,amoebae}.
The measure $\mu$ must furthermore be in a rough phase, meaning that
it is not the restriction of a non-gradient Gibbs measure
to the $\sigma$-algebra $\mathcal F^\nabla$.
It is due to \cite{SHEFFIELD} that the uniqueness statement extends to
any dimension $d\geq 2$,
at least when $s(\mathbf g_i)$ is irrational
for some $1\leq i\leq d+1$.
The rational case is open.
Moreover, it is conjectured in \cite{Linde} that the ergodic
gradient Gibbs measures must be in a smooth phase
in any dimension $d\geq 3$, meaning that those measures are restrictions of non-gradient Gibbs measures.

\subsubsection*{Is $\sigma$ differentiable on the interior of the set of slopes?}
An analytic expression for $\sigma$ is known due to the Kasteleyn theory in dimension $d=2$.
The same route does not---by the knowledge of the author---yield a closed-form
solution for the surface tension in dimension $d\geq 3$.
% Continuity of $\sigma$ is known by Corollary~\ref{corr_sigma_cts}.
It is an open problem to determine if $\sigma$
is differentiable on the interior of $\mathcal S$
in any dimension other than $d=2$.


==> sections/20_introduction_alt.tex <==
%!TEX root= ../main.tex

\section{Height functions on the simplicial lattice}
\label{sec:this_is_the_real_hf_section}

In this section we define the height functions that
are the samples of the model.
We also derive some of their basic properties.

\subsection{The simplicial lattice}
Throughout this paper, $d\geq 2$ denotes a fixed dimension.
Write $\{\mathbf e_i:1\leq i\leq d+1\}$ for the standard basis of $\mathbb R^{d+1}$,
and let $\mathbf n$ denote the vector $\mathbf e_1+\dots+\mathbf e_{d+1}$.
The simplicial lattice is obtained from the square lattice $\mathbb Z^{d+1}\subset\mathbb R^{d+1}$
by identifying vertices that differ by an integer multiple of $\mathbf n$.
In order to formalise the construction, we write $H$ for the orthogonal complement of $\mathbf n$---a $d$-dimensional subspace of $\mathbb R^{d+1}$---and $P:\mathbb R^{d+1}\to H$ for orthogonal projection onto $H$.
Remark that $H$ is precisely the set of vectors in $\mathbb R^{d+1}$ whose coordinates sum to zero.
Let $\{\mathbf g_i:1\leq i\leq d+1\}\subset H$ denote the projection
of the original standard basis,
and note that $\mathbf g_i=\mathbf e_i-\mathbf n/(d+1)$.

\begin{definition}
  \label{def:simpl_latt}
  Write $(X^d,E^d)$ for the projection of the square lattice $\mathbb Z^{d+1}$
  along $P$.
  The graph $(X^d,E^d)$ is called the \emph{simplicial lattice}.
  The $2d+2$ neighbours of a vertex $\mathbf x\in X^d$ are all of the form $\mathbf x\pm\mathbf g_i$.
\end{definition}

\begin{remark}
  \label{remark:presentationinsectionone}
The previous construction is geometric in nature, and one could equally well
define the same graph in a more abstract fashion.
Clearly $(X^d,E^d)$ is graph isomorphic to the Cayley graph of
the Abelian group on $d+1$ generators subject only to
the extra relation that tells us that the product of all $d+1$ generators
produces the identity element of the group.
An alternative presentation of the group $(X^d,+)$ will be of use to us in the proof of Lemma~\ref{lem:cons}.
The embedding of the graph $(X^d,E^d)$ in the vector space $H$
however
makes it easier to work in the geometric setting in Section~\ref{sec:stepped_surfaces}
and to scale height functions in Section~\ref{sec:Statement of the variational principle}.
\end{remark}

\subsection{Height functions}
\begin{definition}\label{hfdefi}
  A \emph{height function}
  is a map $f$ from $X^d$ to $\mathbb R$ that maps $\mathbf 0$ into $(d+1)\mathbb Z$
  and satisfies
  \begin{equation}
    \label{hfdef}
    \nabla f(\mathbf x,\mathbf x+\mathbf g_i):=f(\mathbf x+\mathbf g_i)-f(\mathbf x)\in\left\{1,-d\right\}
  \end{equation}
  for any $\mathbf x\in X^d$ and $1\leq i\leq d+1$.
  Write $\Omega$ for the set of height functions.
  Define
  \begin{equation}
    \label{pointsabovefunction}
    V(f):=\big\{\mathbf x+f(\mathbf x)\mathbf n/(d+1):\mathbf x\in X^d\big\}\subset \mathbb R^{d+1}.
  \end{equation}
  for each $f\in\Omega$.
\end{definition}

By $\nabla f$ we mean the \emph{gradient}
of $f$, that is, the function which takes as its argument a directed edge of
the graph $(X^d,E^d)$
and returns the difference of $f$ along that edge: $\nabla f(\mathbf x,\mathbf x\pm\mathbf e_i):=f(\mathbf x\pm\mathbf e_i)-f(\mathbf x)$ for any $\mathbf x\in X^d$, $1\leq i\leq d+1$.
Obviously $\nabla f$ is antisymmetric: $f(\mathbf x,\mathbf y)+f(\mathbf y,\mathbf x)=0$
whenever $\{\mathbf x,\mathbf y\}\in E^d$.

Informally, we think of the set $V(f)$ as the graph of $f$,
as there exists a linear isomorphism $A$ from
$H\times \mathbb R$ to $\mathbb R^{d+1}$
such that $V(f)=A(\operatorname{Graph}(f))$ for every height function $f\in\Omega$. In the next section we see that $V(f)$
encodes the boundary of a stepped surface.

\subsection{Parity and Lipschitz functions}

The definition of $\mathbf g_i$ implies that each coordinate of the vector
$\mathbf g_i$ has fractional part $-1/(d+1)+\mathbb Z$.
The vectors $\mathbf g_i$ generate the lattice
$X^d$, and therefore
each vector in $X^d$
enjoys the property that the fractional parts
of its $d+1$ coordinates are the same,
and take values in $(\mathbb Z/(d+1))/\mathbb Z$.
Define $\operatorname{Parity}(\mathbf x):=(d+1)(-\mathbf x_1+\mathbb Z)\in \mathbb Z/(d+1)\mathbb Z$, the \emph{parity} of the vertex $\mathbf x\in X^d$.
Let $f\in\Omega$.
The definition of a height function requires that $f(\mathbf 0)\in \operatorname{Parity}(\mathbf 0)=(d+1)\mathbb Z$.
Equation~\ref{hfdef} implies inductively that
$f(\mathbf x)\in \operatorname{Parity}(\mathbf x)$
for all $\mathbf x\in X^d$.


Define the asymmetric norm $\|\cdot\|_+$ on $H$ by
$\|\mathbf x\|_+:=-(d+1)\min_i \mathbf x_i$.
% The asymmetric norm $\|\cdot\|_+$ induces a quasimetric $d_+$ on $H$
% by setting
% $d_+(\mathbf x,\mathbf y):=\|\mathbf y-\mathbf x\|_+$.
A real-valued function $f$ on a subset of $H$
is called \emph{Lipschitz} if
$f(\mathbf y)-f(\mathbf x)\leq\|\mathbf y-\mathbf x\|_+$
for any $\mathbf x$ and $\mathbf y$ in the domain of $f$.
% Now $\|\cdot\|_+$ is the smallest asymmetric norm on $H$
% subject to $\|\mathbf g_i\|_+=1$.
% This implies that $d_+$ takes integral values on $X^d\times X^d$.
It is straightforward to prove following assertion:
if $\mathbf x,\mathbf y\in X^d$, then $\|\mathbf y-\mathbf x\|_+$
denotes the length of the shortest path from $\mathbf x$ to $\mathbf y$
through $(X^d,E^d)$
such that every increment of the path is of the form $\mathbf g_i$; no increments of the form $-\mathbf g_i$ are allowed.
If $f$ is a height function then $f(\mathbf x+\mathbf g_i)-f(\mathbf x)\leq 1$
and inductively $f(\mathbf y)-f(\mathbf x)\leq\|\mathbf y-\mathbf x\|_+$;
each height function must be Lipschitz.
On the other hand, if some $f:X^d\to \mathbb R$ is Lipschitz,
then
\[f(\mathbf x+\mathbf g_i)-f(\mathbf x)\in [-\|-\mathbf g_i\|_+ , \|\mathbf g_i\|_+]=[-d,1].\]
Thus, to check that an arbitrary function $f:X^d\to\mathbb R$ is a height function,
it suffices to check
that $f$ is Lipschitz
and that $f(\mathbf x)\in\operatorname{Parity}(\mathbf x)$
for any $\mathbf x\in X^d$.
The parity condition implies that
the difference in the display
takes as its value one of the two extrema of the interval,
and that $f(\mathbf 0)\in\operatorname{Parity}(\mathbf 0)=(d+1)\mathbb Z$.

\begin{lemma}
  \label{lemma:HFisLIP}
   A function $f:X^d\to\mathbb R$ is a height function if and only if
      $f$ is Lipschitz and $f(\mathbf x)\in\operatorname{Parity}(\mathbf x)$
      for every $\mathbf x\in X^d$.
    If a function $f:H\to\mathbb R$ is Lipschitz then there exists
      a unique largest height function $g$ subject to $g\leq f|_{X^d}$;
      the value of $g$ at each
       $\mathbf x\in X^d$ is given by $g(\mathbf x):=\operatorname{Parity}(\mathbf x)+(d+1)k$,
      where $k\in\mathbb Z$ is maximal subject to $g(\mathbf x)\leq f(\mathbf x)$.
      % Similarly there exists a unique smallest height function $h$
      % subject to $h\geq g|_{X^d}$, and its function values are given by a similar relation.
\end{lemma}

If $f:H\to\mathbb R$ is a Lipschitz function,
then write $\lfloor f\rfloor$ for the largest height function subject to $\lfloor f\rfloor\leq f|_{X^d}$;
its function values are given by the previous lemma.
The previous lemma results in a discrete analogue of the Kirszbraun theorem for the current setting.

\begin{lemma}
  \label{lem:NEW_Kirszbraun}
If $R\subset H$ and $f:R\to \mathbb R$ is Lipschitz,
then $f$ extends to a Lipschitz function $H\to \mathbb R$.
If $R\subset X^d$ and $f:R\to \mathbb R$ is Lipschitz and satisfies
$f(\mathbf x)\in\operatorname{Parity}(\mathbf x)$
for every $\mathbf x\in R$,
then $f$ extends to a height function.
\end{lemma}

The first assertion is the original Kirszbraun theorem.
For the second assertion, let $R\subset X^d$ and $f:R\to\mathbb R$
be as in the lemma. The function $f$ extends to some Lipschitz function
$g:H\to\mathbb R$ by the Kirszbraun theorem. The previous lemma states that $\lfloor g\rfloor$ is a height function that equals
 $f$ on $R$. This proves the second assertion.


==> sections/30_height_functions_alt.tex <==
%!TEX root= ../main.tex

\section{The geometric motivation: stepped surfaces}
\label{sec:stepped_surfaces}
The purpose of this section is to introduce
stepped surfaces,
and to establish the bijection between the set $\Omega$ of height functions 
and the set of stepped surfaces.
We informally think of a stepped surface as a stack
of hypercubes that represents the corresponding height function.

\subsection{Stepped surfaces}
We introduce some simple technical machinery.
% and say that $\mathbf x$ is (\emph{strictly}) \emph{above} $\mathbf y$ whenever $\mathbf x\geq \mathbf y$
% ($\mathbf x>\mathbf y$).
%
% \begin{itemize}
%   \item
  Extend each (strict) order $*\in\{\leq,<\}$ on $\mathbb R$
  to a (strict) partial order on $\mathbb R^{d+1}$
  by declaring $\mathbf x * \mathbf y $ for $\mathbf x,\mathbf y\in\mathbb R^{d+1}$ if and only if $\mathbf x_i *\mathbf y_i$
  for every $1\leq i\leq d+1$.
  % \item
  Say that a set $A\subset \mathbb R^{d+1}$ is \emph{closed under taking lower elements}
  if $\mathbf y\in A$ whenever $\mathbf y\in\mathbb R^{d+1}$
  and $\mathbf y\leq \mathbf x$ for some $\mathbf x\in A$.
  % \item
  Write $L(A)$ for the smallest subset of $\mathbb R^{d+1}$
  that contains $A$ and is closed under taking lower elements;
  this is equivalent to defining $L(A):=\cup_{\mathbf x\in A}\{\mathbf y\in\mathbb R^{d+1}:\mathbf y\leq\mathbf x\}$.
  % \item
  Abbreviate $L(\{\mathbf x\})$ to $L(\mathbf x)$ for $\mathbf x\in\mathbb R^{d+1}$.
  % \item
  Call two elements $\mathbf x,\mathbf y\in \mathbb R^{d+1}$
  \emph{incomparable}
  if neither $\mathbf x< \mathbf y$
  nor  $\mathbf y<\mathbf x$.
  %,
  %in which case we write $\mathbf x\diamond \mathbf y$.
% \end{itemize}


\begin{definition}
  A \emph{stepped surface} is a nonempty strict subset
  of $\mathbb R^{d+1}$
  of the form $L(A)$
  for some $A\subset\mathbb Z^{d+1}$.
  Let $\Psi$ denote the set of stepped surfaces
  and write $V(F)$ for $\partial F\cap\mathbb{Z}^{d+1}$ for any $F\in\Psi$.
\end{definition}

Informally, a stepped surface is a union of ``properly stacked'' unit hypercubes with integral vertices such that there is no ``overhang''.
If $d=2$ then the hypercubes are regular cubes;
 Figure~\ref{fig:2d}\ref{fig:2d:geo} on Page~\pageref{fig:2d} gives an example of such a stepped surface.
If a hypercube is present at the coordinate $\mathbf x$,
then we also require a hypercube to be present at $\mathbf x-\mathbf e_i$
for every $1\leq i\leq d+1$.
This ensures that every hypercube is well-supported, and excludes the possibility of overhang.

There is an obvious bijection from the set $\Psi$ of stepped surfaces
to a set of monotonic functions.
Call a function $m:\mathbb Z^d\to\mathbb Z\cup\{-\infty,\infty\}$ \emph{monotonic}
if it is non-increasing in every coordinate and if $m$
is not identically $-\infty$ or $\infty$.
The monotonic function $m$ associated with
a stepped surface $F\in\Psi$ is given by
the map
$
  \mathbb Z^d\to\mathbb Z\cup\{-\infty,\infty\},\,\mathbf x\mapsto \sup\{k\in\mathbb Z:(\mathbf x,k)\in F\}$.
  The model may thus also be seen as a model of
  discrete monotonic functions.
  The bijection from $\Omega$ to $\Psi$ however is more useful for the analysis.

\begin{theorem}\label{discreteVersionOfPhi}
  The map $\Xi:\Omega\to\Psi,\,f\mapsto L(V(f))$ is a bijection and satisfies $V(\Xi(f))=V(f)$.
\end{theorem}

\begin{proof}
The theorem follows from a series of small intermediate results.
\begin{enumerate}
  \item \emph{If $f\in\Omega$, then $V(f)\subset\mathbb Z^{d+1}$.}
    For this to hold true, it is required that
    \[\mathbf x + f(\mathbf x)\mathbf n/(d+1)\in\mathbb Z^{d+1}\]
    for every $\mathbf x\in X^d$. This follows from
    $f(\mathbf x)\in\operatorname{Parity}(\mathbf x)$
    and the definition of $\operatorname{Parity}(\mathbf x)$.
  \item \emph{If $f\in\Omega$, then any two elements of $V(f)$ are incomparable.}
  Let us pick two elements $\mathbf x,\mathbf y\in X^d$;
  the goal is to prove that the elements in $V(f)$ corresponding
  to $\mathbf x$ and $\mathbf y$ are incomparable.
  It suffices to show that $(\mathbf y+f(\mathbf y)\mathbf n/(d+1))\not<(\mathbf x+f(\mathbf x)\mathbf n/(d+1))$ by symmetry,
  and we may
  assume that $\mathbf y=\mathbf 0$ and $f(\mathbf y)=0$ without loss of generality.
  We thus need to prove that
  $\mathbf 0\not<(\mathbf x+f(\mathbf x)\mathbf n/(d+1))$.
  As $f$ is Lipschitz and $f(\mathbf 0)=0$,
  we have $f(\mathbf x)\leq \|\mathbf x\|_+=-(d+1)\min_i \mathbf x_i$.
  Consequently
  \[\min_i(\mathbf x+f(\mathbf x)\mathbf n/(d+1))_i=\min\nolimits_i\mathbf x_i+f(\mathbf x)/(d+1)\leq 0,\]
  which implies that $\mathbf 0\not<(\mathbf x+f(\mathbf x)\mathbf n/(d+1))$.
\end{enumerate}

Fix $f\in\Omega$ and $\mathbf x\in V(f)$,
and claim that $\mathbf x\in \partial L(V(f))$.
Suppose that $\mathbf x\not\in\partial L(V(f))$.
Then $\mathbf x<\mathbf y$ for some $\mathbf y\in L(V(f))$,
and therefore $\mathbf x<\mathbf z$ for some $\mathbf z\in V(f)$.
This contradicts that any two elements of $V(f)$ are incomparable and proves the claim.
Conclude that $V(f)\subset \partial L(V(f))$.

Consider the set $L(V(f))$. This must be
a stepped surface, as it has nonempty boundary (and is therefore a strict nonempty subset of $\mathbb R^{d+1}$) and because $V(f)\subset \mathbb Z^{d+1}$.
Conclude that the map $\Xi$ is well-defined, and satisfies
$V(f)\subset V(\Xi(f))$ for every $f\in\Omega$.

\begin{enumerate}[resume]
  \item \emph{If $F\in\Psi$, then $F$ is closed,
  and if $\mathbf x\in \partial F$, then one of the coordinates of $\mathbf x$ is integral.}
  Fix $F\in\Psi$, and choose $A\subset\mathbb Z^{d+1}$
  such that $F=L(A)$.
  If $\mathbf x\in A$, then $L(\mathbf x)$ is a union
  of closed unit hypercubes with integral vertices.
  Therefore $F=\cup_{\mathbf x\in A}L(\mathbf x)$
  is a union of closed unit hypercubes with integral vertices.
  Locally this union reduces to a finite union;
  the claim is now readily verified.
  \item \emph{The projection map $P$ restricts to a bijection from $V(F)$ to $X^d$.}
  Clearly $PV(F)\subset P\mathbb Z^d =X^d$.
  Fix $\mathbf x\in X^d$, and let us look at the set
  $(P|_{\partial F})^{-1}(\mathbf x)=(\mathbf x+\mathbb R\mathbf n)\cap \partial F$.
  The line $\mathbf x+\mathbb R\mathbf n$ intersects
  both $F$ and its complement (as $F$ is closed under taking lower elements, and because $F$ is nonempty nor equals $\mathbb R^{d+1}$).
  In particular, the previous intersection is nonempty; say it contains some element
  $\mathbf y$.
  If the intersection contains another elements, say $\mathbf z$,
  then either $\mathbf z<\mathbf y$ or $\mathbf y<\mathbf z$
  (as $<$ reduces to a total strict order on the line)
  and therefore one of the two must be contained in the interior
  of $F$ (as $F$ is closed under taking lower elements), a contradiction.
  The element $\mathbf y$ is thus the only point of intersection.
  By the previous result, one of the coordinates of $\mathbf y$ must be integral.
  But then all coordinates of $\mathbf y$ must be integral,
  as each element of $X^d+\mathbb R\mathbf n=\mathbb Z^{d+1}+\mathbb R\mathbf n$ enjoys the property
  that the fractional parts of its coordinates are equal.
  Conclude that $\mathbf y\in\mathbb Z^{d+1}$,
  and therefore $(P|_{V(F)})^{-1}(\mathbf x)=\{\mathbf y\}$.
\end{enumerate}

We had already seen that $\Xi(f)\in\Psi$
and that $V(f)\subset V(\Xi(f))$.
The fourth result in the series tells us that
 $V(\Xi(f))$ cannot contain any more elements than necessary for this inclusion, that is, $V(f)= V(\Xi(f))$.
The assignment $f\mapsto V(f)$ is injective,
 and therefore the map $\Xi$ must also be injective.
It suffices to show that the map $\Xi$ is surjective.
It is straightforward to demonstrate that the inverse map is given by
\[\Xi^{-1}(F):X^d\to\mathbb R,\,\mathbf x\mapsto \max\{a\in\mathbb R:\mathbf x+a\mathbf n/(d+1)\in F\}.\]
This proves the theorem.
\end{proof}


\subsection{The map $\Xi$ preserves the order}
The map $\Xi$ is an order-preserving bijection from $(\Omega,\leq)$ to $(\Psi,\subset)$.
Moreover, taking the pointwise maximum of two height functions
is equivalent to taking
the union of the corresponding stepped surfaces.
Taking the pointwise minimum corresponds to taking an intersection.
This is summarised in the following proposition.

\begin{proposition}
  \label{pro:aux}
  Let $f_1$ and $f_2$ be height functions and let $F_1=\Xi(f_1)$ and $F_2=\Xi(f_2)$.
  Then
  \begin{enumerate}
    \item\label{pro:aux:orderwell} $f_1\leq f_2$ if and only if $F_1\subset F_2$,
    \item $f_1\vee   f_2$ is a height function,
    $F_1\cup F_2$ is a stepped surface, and $\Xi(f_1\vee f_2)=F_1\cup   F_2$, \label{pro:aux_1}
    \item $f_1\wedge f_2$ is a height function, $F_1\cap F_2$ is a stepped surface, and $\Xi(f_1\wedge f_2)=F_1\cap F_2$. \label{pro:aux_2}
  \end{enumerate}
\end{proposition}

Of course,~\ref{pro:aux_1} and~\ref{pro:aux_2} extend to finite unions, intersections, maxima, and minima.

\subsection{Local moves}\label{subsec:localmove}
If two height functions differ at only finitely many points,
then the first may be transformed into the second by changing the value of the height function
at one vertex at a time.
All intermediate functions must also be height functions.
The operation of changing the value of a height function at a single vertex
is called a \emph{local move}.
A local move is equivalent to adding or removing a single unit hypercube to the corresponding stepped surface.

\begin{lemma}
  \label{lem:localMove}
  Suppose that $R\subset X^d$ is finite
  and that $f$ and $g$ are height functions that are equal outside
  $R$ and satisfy $f\leq g$ on $R$.
  Then there exists a sequence of height functions
  $(f_k)_{0\leq k\leq n}\subset \Omega$
  with
  \begin{enumerate}
    \item $f_0=f$ and $f_n=g$,
    \item for every $0\leq k<n$ there exists a unique
    $\mathbf x\in R$ such that
    $f_{k+1}=f_k+(d+1)\cdot 1_{\mathbf x}$.
  \end{enumerate}
  Note that the sequence is automatically increasing and all functions agree
  to $f$ and $g$ outside of $R$.
\end{lemma}

\begin{proof}
We induct on the number $N(f,g):=\sum_{\mathbf x\in R}(g(\mathbf x)-f(\mathbf x))$.
Clearly the length of the sequence must be $n=N(f,g)/(d+1)$.
Set $f_0=f$. To start the induction it is sufficient to find an appropriate vertex
$\mathbf x\in R$ at which to increase $f_0$ to obtain a new function $f_1$.
Define $S=\{\mathbf x\in R:f(\mathbf x)<g(\mathbf x)\}$.
Clearly the point $\mathbf x$ must be chosen from $S$.
Now pick $\mathbf x\in S$ to minimise $f(\mathbf x)$.
It is straightforward to prove that $\mathbf x$ is a local minimum of $f$,
in the sense that
$\nabla f (\mathbf x,\mathbf x+\mathbf g_i)=1$
and $\nabla f (\mathbf x,\mathbf x-\mathbf g_i)=d$ for all $1\leq i\leq d+1$.
Conclude that $f_1=f_0+(d+1)\cdot 1_{\mathbf x}$ is the desired function.
\end{proof}

If $f$ and $g$ agree outside $R$ but neither $f\leq g$ nor $f\geq g$,
then one can first go down from $f$ to $f\wedge g$ and then up from $f\wedge g$
to $g$. Proposition~\ref{pro:aux} ensures that $f\wedge g$ is a height function.


==> sections/40_simplicial_lattice.tex <==
%!TEX root= ../main.tex
\section{The simplicial lattice and tilings}
\label{sec:simplicial_lattice}

In this section we explore the simplicial lattice.
% From now on $d\geq 2$.
In dimension $d=2$ the graph $(X^d,E^d)$ is the triangular lattice; see Figure~\ref{fig:2d}\ref{fig:2d:hf}.
The paths of length $3$ that traverse triangles
are in some sense the building blocks for all closed walks through the triangular lattice.
One goal of this section is to formalise and generalise this claim, in Lemma~\ref{lem:cons}.
In Subsection~\ref{subsec:tilings} we define tilings, which generalise the lozenge tilings
of Figure~\ref{fig:2d}\ref{fig:2d:geo}.
% In the last subsection we introduce a hypergraph that is dual
% to $(X^d,E^d)$. The dual hypergraph turns out to be fundamental for the development of the
% Kasteleyn theory in Section~\ref{}.

\subsection{Simplicial loops}

We first define simplicial loops, which generalise paths along triangles
through the triangular lattice.
Observe that, in any dimension $d$,
\[\mathbf g_1+\dotsb+\mathbf g_{d+1}=P\mathbf e_{1}+\dotsb+P\mathbf e_{d+1}=P\mathbf n=\mathbf 0.\]
This means that if a path through the simplicial lattice $(X^d,E^d)$ is of length $d+1$
and has increments $\{\mathbf g_1,\dots,\mathbf g_{d+1}\}$,
then it is automatically closed.
We call such paths \emph{simplicial loops}.

\begin{definition}
  \label{sldef}
  A path $(\mathbf s_k)_{0\leq k\leq d+1}\subset X^d$ of length $d+1$ is called a \emph{rooted simplicial loop}
  or simply a \emph{simplicial loop}
  if there exists a permutation $\xi\in S_{d+1}$ such that
  $\mathbf s_k=\mathbf s_{k-1}+\mathbf g_{\xi(k)}$ for any $1\leq k\leq d+1$.
  Write $R^d$ for the set of rooted simplicial loops.
  Sometimes we are not concerned with the starting points of the loops.
  In those cases, two loops are considered equal if they are equal up to indexation---this is equivalent to requiring that the two loops traverse the same set of edges.
  Write $U^d$ for the set of \emph{unrooted simplicial loops}.
\end{definition}

\subsection{Conservative flows}

In this subsection we show that simplicial loops are the building blocks for
all closed walks through $(X^d,E^d)$.
This result is proven in terms of flows; we first introduce some standard terminology.
Write $\vec E^d$ for the directed edges of $(X^d,E^d)$,
that is,
$\vec E^d:=\{(\mathbf x,\mathbf y)\in X^d\times X^d:\{\mathbf x,\mathbf y\}\in E^d\}$.
A \emph{flow} is a function
$\alpha:\vec E^d\to\mathbb R$
that is antisymmetric under interchanging the two arguments.
If $\mathbf p=(\mathbf p_k)_{0\leq k\leq n}$ is a walk through $(X^d,E^d)$
and $\alpha$ a flow, then write
\[{\int_{\mathbf p}\alpha} :=\sum_{k=1}^{n}\alpha(\mathbf p_{k-1},\mathbf p_k).\]
A flow $\alpha$ is called \emph{conservative} if $\int_\mathbf p\alpha=0$
for every closed walk $\mathbf p$.
If $\alpha$ is conservative, then write
\[\int_{\mathbf x}^{\mathbf y}\alpha:=\int_\mathbf p\alpha\]
for any $\mathbf x,\mathbf y\in X^d$, where $\mathbf p$ is a walk from $\mathbf x$
to $\mathbf y$.
The choice of the walk does not matter, precisely because $\alpha$ is conservative.
Conservative flows are also called \emph{gradient flows}.
If $f:X^d\to \mathbb R$ then the flow
$\nabla f$ is conservative,
and $\int_\mathbf x^\mathbf y\nabla f=f(\mathbf y)-f(\mathbf x)$.

\begin{lemma}
\label{lem:cons}
Let $\alpha$ be a flow on $(X^d,E^d)$.
Suppose that $\int_{\mathbf s}\alpha=0$ for every simplicial loop $\mathbf s\in R^d$.
Then the flow $\alpha$ is conservative.
\end{lemma}

\begin{proof}
  Write $G:=\{\mathbf g_1,\dots,\mathbf g_{d+1}\}$.
  We desribe two presentations of the group $(X^d,+)$ that have
   generating set $G$---the difference is thus
   in the choice of relators.
  Write $C$ for set
  of commutators of pairs of generators,
  that is, the set of relators of the form
  $(\mathbf g_i,\mathbf g_j,-\mathbf g_i,-\mathbf g_j)$.
  Define $R_1:=C\cup\{(\mathbf g_1,\dotsb,\mathbf g_{d+1})\}$.
  It was observed in Remark~\ref{remark:presentationinsectionone}
  that $(X^d,+)=\langle G| R_1\rangle$.
  Write $R_2$ for the set of relators
  \[R_2=\left\{\left(\mathbf g_{\xi(1)},\dots,\mathbf g_{\xi(d+1)}\right):\xi\in S_{d+1}\right\}.\]
  Each relator in $R_2$ sums to $\mathbf 0$ in
  the group $(X^d,+)$,
  and one can show that the group $\langle G|R_2\rangle$ is commutative.
  Conclude that
  $(X^d,+)=\langle G| R_1\rangle=\langle G| R_2\rangle$.

  The graph $(X^d,E^d)$ is the Cayley graph of the group $(X^d,+)$ with generators $G$.
  To check that a flow $\alpha$ on such a Cayley graph is conservative,
  it suffices to check that $\int_\mathbf p\alpha=0$ for any
  closed walk $\mathbf p$ whose increments are given by a relator.
  If we choose the set $R_2$ for the set of relators,
  then the set of such closed walks is precisely the set of simplicial loops.
\end{proof}

\subsection{Tilings}\label{subsec:tilings}

Consider a height function $f$ and a simplicial loop $\mathbf s$.
By Definition~\ref{hfdefi}, $\nabla f(\mathbf s_{k-1},\mathbf s_k)$
takes values in $\{1,-d\}$.
Since $\nabla f$ is conservative, there is a unique
$k$ such that $\nabla f(\mathbf s_{k-1},\mathbf s_k)=-d$,
and $\nabla f$ equals $1$ along all other directed edges of $\mathbf s$.
Introduce the following notation.

\begin{definition}
  \label{def:alpha}
  For any $f\in\Omega$, define
   $\Phi(f):=(f(\mathbf 0),T(f))$ where \[T(f):=\{\{\mathbf x,\mathbf x+\mathbf g_i\}\in E^d:\nabla f(\mathbf x,\mathbf x+\mathbf g_i)=-d\}\subset E^d.\]
  For any $T\subset E^d$, define the flow $\alpha_T$ on $(X^d,E^d)$ by
  \[\alpha_T(\mathbf x,\mathbf x+\mathbf g_i):=\begin{cases}
    -d &\text{if $\{\mathbf x,\mathbf x+\mathbf g_i\}\in T$},\\
    1 &\text{if $\{\mathbf x,\mathbf x+\mathbf g_i\}\not\in T$},
  \end{cases}\]
  and note that $\alpha_{T(f)}=\nabla f$.
\end{definition}

Every simplicial loop contains exactly one edge of $T(f)$, by the previous discussion.
Now suppose that we start with another set $T\subset E^d$ with the quality
that every simplicial loop contains exactly one edge of $T$.
Then $\int_\mathbf s\alpha_T=0$ for every simplicial loop $\mathbf s$,
and therefore Lemma~\ref{lem:cons} tells us that $\alpha_T$ is conservative.
In particular, we can define the function
$X^d\to\mathbb R,\,\mathbf x\mapsto \int_\mathbf 0^\mathbf x \alpha$,
and this is a height function that maps $\mathbf 0$ to $0$.

\begin{definition}
  \label{def:tilings}
  A set $T\subset E^d$ is called a \emph{tiling} if every simplicial loop contains exactly one edge of $T$.
  Write $\Theta$ for the set of tilings.
\end{definition}

\begin{theorem}
  \label{thm:bijectionOmegTheta}
  The map $\Phi:\Omega\to (d+1)\mathbb Z\times\Theta$ is a bijection with inverse \[\textstyle (a,T)\mapsto \left(X^d\to\mathbb R,\,\mathbf x\mapsto a+\int_\mathbf 0^\mathbf x\alpha_T\right).\]
\end{theorem}

\begin{remark}
  A set $T\in\Theta$ is not a tesselation of $H\cong\mathbb R^d$ in the spirit of Figure~\ref{fig:2d}\ref{fig:2d:geo}: it is merely a collection of edges.
  The formulation of Definition~\ref{def:tilings} is combinatorial and convenient in the setting of this article.
  One can also generalise the geometrical picture of Figure~\ref{fig:2d}\ref{fig:2d:geo}.
  Suppose that we aim to construct the tesselation of $H$ corresponding to a cubic profile $F\in\Psi$.
  Its topological boundary $\partial F$ should be thought of as a collection of hypercubes of
  dimension $d$---and thus of
  codimension one relative to the ambient space $\mathbb R^{d+1}$
  that the stepped surface $F$ lives in.
  One can simply project each of these hypercubes down onto $H$ with the projection $P$.
  This construction is clearly invariant under translating $F$ by (integer multiples of) $\mathbf n$.
  The collection of projected codimension-$1$ hypercubes
  partitions the space $H$ up to the overlapping boundaries of the tiles,
  because $P$ restricts to a bijection from $\partial F$
  to $H$. (This is similar to the fourth intermediate result of the proof of Theorem~\ref{discreteVersionOfPhi}.)
  The tiles of the tesselation associated with $F$
  are in bijection with the edges of $T(F)$;
  each edge in $T(F)$ is contained in exactly one
  tile of the tesselation, and this correspondence is bijective.
\end{remark}

